SCALE-Sim v3: A modular cycle-accurate systolic accelerator simulator for end-to-end system analysis

The rapid advancements in AI, scientific computing, and high-performance computing (HPC) have driven the need for versatile and efficient hardware accelerators. Existing tools like SCALE-Sim v2 provide valuable cycle-accurate simulations for systolic-array-based architectures but fall short in supporting key modern features such as sparsity, multi-core scalability, and comprehensive memory analysis. To address these limitations, we present SCALE-Sim v3, a modular, cycle-accurate simulator that extends the capabilities of its predecessor. SCALE-Sim v3 introduces five significant enhancements: multi-core simulation with spatio-temporal partitioning and hierarchical memory structures, support for sparse matrix multiplications (SpMM) with layer-wise and row-wise sparsity, integration with Ramulator for detailed DRAM analysis, precise data layout modeling to minimize memory stalls, and energy and power estimation via Accelergy. These improvements enable deeper end-to-end system analysis for modern AI accelerators, accommodating a wide variety of systems and workloads and providing detailed full-system insights into latency, bandwidth, and power efficiency. A 128x128 array is 6.53x faster than a 32x32 array for ViT-base, using only latency as a metric. However, SCALE-Sim v3 finds that 32x32 is 2.86x more energy-efficient due to better utilization and lower leakage energy. For EdP, 64x64 outperforms both 128x128 and 32x32 for ViT-base. SCALE-Sim v2 shows a 21% reduction in compute cycles for six ResNet18 layers using weight-stationary (WS) dataflow compared to output-stationary (OS). However, when factoring in DRAM stalls, OS dataflow exhibits 30.1% lower execution cycles compared to WS, highlighting the critical role of detailed DRAM analysis.

==> sections/artifact_evaluation.tex <==
% LaTeX template for Artifact Evaluation V20240722
%
% Prepared by Grigori Fursin with contributions from Bruce Childers,
%   Michael Heroux, Michela Taufer and other colleagues.
%
% See examples of this Artifact Appendix in
%  * ASPLOS'24 "PyTorch 2: Faster Machine Learning Through Dynamic Python Bytecode Transformation and Graph Compilation": 
%      https://dl.acm.org/doi/10.1145/3620665.3640366
%  * SC'17 paper: https://dl.acm.org/citation.cfm?id=3126948
%  * CGO'17 paper: https://www.cl.cam.ac.uk/~sa614/papers/Software-Prefetching-CGO2017.pdf
%  * ACM ReQuEST-ASPLOS'18 paper: https://dl.acm.org/citation.cfm?doid=3229762.3229763
%
% (C)opyright 2014-2024 cTuning.org
%
% CC BY 4.0 license
%


% \special{papersize=8.5in,11in}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% When adding this appendix to your paper, 
% please remove above part
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\appendix
\section{Artifact Appendix}
% \setminted{breaklines, breakanywhere}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}

The artifact appendix section describes how to access the artifacts of the \NAME v3 simulator introduced in \autoref{fig:scalesim v3 overview}. The artifact also describes how to reproduce the experiments in \autoref{sec:mulicore} (\autoref{fig:spatiotemporal}), \autoref{sec:sparsity} (\autoref{fig:sparsity-lws-resnet18-computecyclesplot}, \autoref{fig:sparsity-resnet18-memoryplot}, and  \autoref{fig:sparsity-gemm-computecycles-overlap}), \autoref{sec:ramulator} (\autoref{fig:bw_channel} and \autoref{fig:stall_cycle}), \autoref{sec:layout} (\autoref{fig:result_bandwidth_evaluation} and \autoref{fig:result_bandwidth_evaluation_vit}) conducted through the \NAME v3 framework. 

\subsection{Artifact check-list (meta-information)}

% {\em Obligatory. Use just a few informal keywords in all fields applicable to your artifacts
% and remove the rest. This information is needed to find appropriate reviewers and gradually 
% unify artifact meta information in Digital Libraries.}

{\small
\begin{itemize}
  \item {\bf Program: Python3 and C++11 compiler (e.g., clang++, g++-5)}
  \item {\bf Hardware: Linux-based}
  \item {\bf Metrics: Latency, Memory, Throughput and Energy}
  \item {\bf Output: Compute and Bandwidth csv reports in addition to sparsity report, Ramulator report and Accelergy report}
  \item {\bf How much disk space required (approximately)?: 10 GB}
  \item {\bf How much time is needed to prepare workflow (approximately)?: 5 minutes}
  \item {\bf How much time is needed to complete experiments (approximately)?: 15-20 hours}
  \item {\bf Publicly available?: Yes}
  \item {\bf Code licenses (if publicly available)?: MIT License (LICENCE file in the GitHub repository)}
\end{itemize}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description}

\subsubsection{How to access}

The artifact is uploaded to Zenodo (DOI: 10.5281/zenodo.15170910)
\subsubsection{Hardware dependencies}
The artifact has been tested on Linux-based systems
\subsubsection{Software dependencies}
Python3 and C++11 compiler (e.g., clang++, g++-5)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Installation}
For artifact evaluation, please follow the following steps:
\begin{minted}[fontsize=\footnotesize, frame=single]{bash}
$ git clone 
https://github.com/scalesim-project/scale-sim-v2.git
$ cd scale-sim-v2
$ git checkout v3_artifact
$ pip install -r requirements.txt
$ pip install -e .
$ export PYTHONPATH=.:$PYTHONPATH
\end{minted}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment workflow}
Now that our environment is set up, we will run the SCALE-Sim v3 artifact and evaluate the result. The first step is to write config and topology files. The config and topology files for the experiments are provided under the folder \textit{configs} and \textit{topologies} respectively. In addition, the layout files are provided under the folder \textit{layouts}.

For config file and topology file customization for sparsity, see the Experiment customization section.


To evaluate the experiment more conveniently, we provide python and shell scripts for each part, which will be introduced in the next section.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation and expected results}

\subsubsection{Multi-core (\autoref{fig:spatiotemporal})}
\begin{minted}[fontsize=\footnotesize, frame=single]{bash}
$ python3 multi-core/analytical.py 
$ python3 multi-core/plot_scatter.py
\end{minted}
Figures will be produced in \textit{multi-core} directory named \textit{compute\_optimized\_tradeoff.pdf} and \textit{memory\_optimized\_tradeoff.pdf} reproducing figures \hyperref[fig:spatiotemporal]{3a} and \hyperref[fig:spatiotemporal]{3b} respectively.


\subsubsection{Sparsity (\autoref{fig:sparsity-lws-resnet18-computecyclesplot})}
\begin{minted}[fontsize=\footnotesize, frame=single]{bash}
$ python3 sparsity/compute_cycles_plot_128x128.py 
\end{minted}
A figure will be produced in \textit{sparsity} directory named \textit{resnet18\_compute\_cycles.pdf} reproducing \autoref{fig:sparsity-lws-resnet18-computecyclesplot}.

Please note that the python file plots based on experimental data collected in \textit{sparsity/sparsity\_results\_128x128} folder. To reproduce the experimental data, please follow the \textit{README.md} file in the \textit{sparsity folder}. The expected time to finish all the runs is around 10-12 hours. The same experimental data has been used for the next subsection as well.


\subsubsection{Sparsity (\autoref{fig:sparsity-resnet18-memoryplot}}
\begin{minted}[fontsize=\footnotesize, frame=single]{bash}
$ python3 sparsity/memoryplot.py 
\end{minted}
A figure will be produced in \textit{sparsity} directory named \textit{memoryplot.pdf} reproducing \autoref{fig:sparsity-resnet18-memoryplot}.

\subsubsection{Sparsity (\autoref{fig:sparsity-gemm-computecycles-overlap})}
\begin{minted}[fontsize=\footnotesize, frame=single]{bash}
$ bash sparsity/run_vit_compute.sh
\end{minted}
A figure will be produced in \textit{sparsity} directory named \textit{vit\_compute\_cycles\_scatterplot.pdf} reproducing \autoref{fig:sparsity-gemm-computecycles-overlap}.


\subsubsection{Layout (\autoref{fig:result_bandwidth_evaluation}, \autoref{fig:result_bandwidth_evaluation_vit})}
\begin{minted}[fontsize=\footnotesize, frame=single]{bash}
$ bash layout_plots/run_layout.sh
\end{minted}
Figures will be produced in \textit{layout\_plots} directory named \textit{multi\_bank\_vs\_bandwidth\_model\_resnet18.pdf} and \textit{multi\_bank\_vs\_bandwidth\_model\_vit.pdf} reproducing \autoref{fig:result_bandwidth_evaluation} and \autoref{fig:result_bandwidth_evaluation_vit} respectively.

\subsubsection{Ramulator }

Please follow the given steps:

\begin{minted}[fontsize=\footnotesize, frame=single]{bash}
$ git checkout dev-ramulator-merge
$ pip install -r requirements.txt
$ git submodule update --init --recursive
$ cd submodules
$ cp -r ../scripts/ramulator_patch/* ./ramulator/
$ cd ramulator
$ make -j <num_jobs>
\end{minted}

To reproduce \autoref{fig:bw_channel}, use the following command:
\begin{minted}[fontsize=\footnotesize, frame=single]{bash}
$ cd ../../ 
$ source generate_fig9_ramulator_mem_bw_plot.sh
\end{minted}


To reproduce \autoref{fig:stall_cycle}, use the following command:
\begin{minted}[fontsize=\footnotesize, frame=single]{bash}
$ source generate_fig10_ramulator_stall_plot.sh
\end{minted}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment customization}
To run customized experiments, users can write their own config and topology files and feed it to the program. Let's take sparsity as an example. In a config file, the full list of sparsity parameters include:

\newpage

\begin{minted}[fontsize=\footnotesize, frame=single]{bash}
SparsitySupport : enable or disable sparsity support
SparseRep: sparsity representation (csr, csc,
ellpack_block)
OptimizedMapping : enable row-wise sparsity, 
the default is layer-wise sparsity
BlockSize : M in N:M ratio for row-wise sparsity
\end{minted}

The sparsity topology files look as follows:
\begin{minted}[fontsize=\footnotesize, frame=single]{text}
Layer Name, M, N, K, Sparsity,
GEMM_1, 3, 5, 16, 3:4,
GEMM_2, 1, 5, 16, 1:4,
\end{minted}

where, M, N, and K are regular GEMM dimensions. The entries in \textit{Sparsity} are in the N:M format corresponding to N:M row-wise sparsity.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Notes}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Methodology}

Submission, reviewing and badging methodology:

\begin{itemize}
  \item \url{https://www.acm.org/publications/policies/artifact-review-and-badging-current}
  \item \url{https://cTuning.org/ae}
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% When adding this appendix to your paper, 
% please remove below part
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/combined_studies.tex <==
\section{Studies combining multiple features}

==> sections/verification.tex <==
\section{Verification}
